Cross-validation on Extreme Regions

We conduct a non asymptotic study of the Cross Validation (CV) estimate of the generalization risk for learning algorithms dedicated to extreme regions of the covariates space. In this Extreme Value Analysis context, the risk function measures the algorithm's error given that the norm of the input exceeds a high quantile. The main challenge within this framework is the negligible size of the extreme training sample with respect to the full sample size and the necessity to re-scale the risk function by a probability tending to zero. We open the road to a finite sample understanding of CV for extreme values by establishing two new results: an exponential probability bound on the \Kfold CV error and a polynomial probability bound on the leave-\textrm{p}-out CV. Our bounds are sharp in the sense that they match state-of-the-art guarantees for standard CV estimates while extending them to encompass a conditioning event of small probability. We illustrate the significance of our results regarding high dimensional classification in extreme regions via a Lasso-type logistic regression algorithm. The tightness of our bounds is investigated in numerical experiments.

==> abstract.tex <==
We conduct a non asymptotic study of the Cross Validation (CV) 
 estimate of the generalization risk
for   learning algorithms dedicated
to extreme regions of the covariates space. In this Extreme Value Analysis context,
the risk
function measures the algorithm's error given that the norm of the
input  exceeds a high quantile. The main challenge within
this framework is the negligible size of the extreme training sample
with respect to the full sample size and the necessity to re-scale the
risk function by a probability tending to zero. We open the road to a finite sample understanding of CV for extreme values by establishing two new results: an exponential probability bound on the $K$-fold CV error
and a polynomial probability bound on the leave-$p$-out CV. Our bounds are sharp in the sense that they match state-of-the-art guarantees for standard CV estimates while extending them to encompass a conditioning event of small probability. We illustrate the significance of our results regarding high dimensional classification in extreme regions via a \Lasso-type logistic regression algorithm.   The tightness of our bounds is investigated in numerical experiments.



==> intermediate-mainpaper.tex <==
In this section we gather the main intermediate results involved in the proofs of our main results theorems~\ref{theo:main-sanity-rare} and~\ref{theo:main-sanity-rare-lpo}, which are of interest in their own.


A key tool to our proofs is  a Bernstein-type inequality relative to the deviation of a generic random variable $Z=f(O_1,\ldots,O_n)$ from its mean (\cite{McDiarmid98conc}) that we recall in the supplement for convenience (Proposition~\ref{"Bernstein-extension"}). The control of the deviations involves both a maximum deviation term and a variance term.   We leverage this result to control the deviations of the  pseudo-empirical risk $\tilde \risk_\alpha$ defined in ~(\ref{def:tilde-rcv}) averaged over the $K$ validation sets $V_{1:K}$. These deviations are embodied by the random variable $Z$ defined in Lemma~\ref{"RCV-supp"}, Equation~(\ref{def:Z-CV}), which is a key quantity when analysing the deviations of any \CV risk estimate as revealed by an inspection of the proofs in the supplement.  Controlling the deviations of $Z$ is the main purpose of this section.




\begin{lemma}
	\label{"RCV-supp"}
Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables, and $V_1,V_2,\dots V_K$ a sequence of masks that verifies Assumption~\ref{assum:mask-property} with size $n_V$.\,Moreover,\,suppose that assumptions~\ref{assum:hypo-class} and~\ref{assum:cost-func} regarding the class $\mathcal{G}$ and $c$ hold. Define 

\begin{equation}\label{def:Z-CV}
Z=\ffrac{1}{K}\sum_{j=1}^{K}\sup_{g \in \mathcal{G}}\lvert \Tilde{\mathcal{R}}_{\alpha}(g,V_{j})-\mathcal{R}_\alpha(g) \rvert,
\end{equation}

where $\Tilde{\mathcal{R}}_{\alpha}$ is defined by Equation~\ref{def:tilde-rcv}.\,Then the random variable $Z$  satisfies the Bernstein-type inequality	
\[P\left(Z - E(Z) \geq t  \right)\leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).\]	
\end{lemma}


\begin{proof}
 The reader is referred to Appendix~\ref{"lemma-RCV-supp-proof"}.	
\end{proof}

To obtain a genuine probability bound on $Z$ \emph{via} the latter lemma, one also needs to control the term $E(Z)$. This is the purpose of the next lemma, the spirit of which is similar to Lemma 14 in~\cite{goix15}. The main difference \wrt to the latter reference is that we handle any bounded cost function (not only the Hamming loss), using a bound for Rademacher averages from~\cite{gine2001consistency} which applies in this broader setting.
\begin{lemma}
	\label{"RCV-expectation"}

        In the setting of Lemma~\ref{"RCV-supp"}, $Z$ satisfies %we have
        \[
	\EE(Z) \leq   \ffrac{M\sqrt{\vapnikG}}{\sqrt{\alpha n_V}}.
	\]
 
where $M>0$ is a universal constant. % some constant $M>0$.
\end{lemma}

\begin{proof}	
	See Appendix~\ref{"proof-RCv-expectation"}
\end{proof}

The following probability upper bound for $Z$ follows immediately by combining Lemma~\ref{"RCV-supp"} and Lemma~\ref{"RCV-expectation"}. % the following corollary. 
\begin{corollary}
	\label{"RCV-sup-control"}
        In the setting of Lemma~\ref{"RCV-supp"}, 

        we have
	\[P\left(Z - \ffrac{M\sqrt{\vapnikG}}{\sqrt{\alpha n_V}}\geq t \right)\leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right),\]
	where $Z$ is defined in \eqref{def:Z-CV}.
\end{corollary}



==> intermediate.tex <==
This section gathers generic concentration tools and technical intermediate results that are necessary to the proofs of our main results. %\,we introduce some intermediate results that will be used in this paper.

\subsection{Generic tools}
\label{sec:genericTools}


\,First,\,we recall the following McDiarmid's extension of Bernstein inequality (Theorem 3.8 in \cite{McDiarmid98conc}).
\begin{proposition}\label{"Bernstein-extension"}
	For a sequence of observations $(O_1,O_2,\dots,O_n) \in \mathcal{Z}^n$ and some fixed values $o_{1:l}=(o_1,o_2,\dots,o_l)$ and for some measurable function $f\,:\,\mathcal{Z}^n\rightarrow \rset$,\,let $Z=f(O_1,O_2,\dots,O_n)$ and define for $l \in \llbracket1,n\rrbracket$:
	\begin{enumerate}
		\item $f_{l}(o_1,o_2,\dots,o_l)=\mathbb{E}\left (Z \mid O_1=o_1,O_2=o_2,\dots,O_l=o_l\right),$ 
		\item $\Delta_l(o_1,o_2,\dots,o_{l-1},o_l)  =f_{l}(o_1,o_2,\dots,o_{l-1},o_l)-f_{l-1}(o_1,o_2\dots,o_{l-1}),$ (the positive deviations)
		\item $D:=\max _{l=1, \ldots, n} \sup _{o_{1}, \ldots, o_{i-1} \in \mathcal{X}} \sup _{o \in \mathcal{X}} \Delta_{l}\left(o_{1}, \ldots, o_{l-1}, o\right),$ (the maximum positive deviation)
		\item  $\sigma_{l}^2(o_{1:l-1})=\Var\left[ \Delta_l(O_1,O_2,\dots,O_{l-1},O' ) 
		\mid O_1=o_1, O_2=o_2 , \dots , O_{l-1}=o_{l-1} \right],$ where $O'$ is an independent copy of $O_1,$
            \item
              $\sigma^2=\sum_{l=1}^n \sup_{o_{1:l-1}\in
                \mathcal{X}^{l-1}} \sigma^2_l(o_{1:l-1})$ (the
              maximum sum of variances).
	\end{enumerate}
	Then we have
	\[ \PP(Z - \EE[Z] > t ) \le \exp{\left(\ffrac{-t^2}{2(\sigma^2 + Dt/3)}\right)}. \]
      \end{proposition}


We also recall Proposition 2.5.2 from \cite{vershynin_2018},\,which provides an upper bound for the expectation of sub-Gaussian random variables.
\begin{proposition}\label{"Expectation-UB-subgauss"}
Let $X$ be a real valued random variable and suppose that $$\PP(X\geq t)\leq C_1\exp{\left(-t^2/C_2^2\right)},$$ for some $C_1 , C_2 > 0$, then there exists a constant $M_2>0$ which depends only on $C_1$,\,such that
\[ \EE(X) \leq M_2 C_2.
\] 
\end{proposition}

      
%\vspace{10mm}
%In addition,\,to show the desired results,\,one need to make the following assumption :
%\begin{assumption}[mask property]\label{assum:mask-property}
%	The sequence of masks $S_1,S_2,\dots S_K$  verifies :
%	\begin{equation}\label{"card-condition"}
%	card(S_j)=n_S\quad \forall j \in \llbracket1,K\rrbracket
%	\end{equation}
%	for some $n_S \in \llbracket1,n\rrbracket$.\,Moreover :
%	\begin{equation}\label{"key-condition"}
%	\frac{1}{K}\sum_{j=1}^{K}\ffrac{\indic{l \in S_j} }{n_S}=\frac{1}{n} \quad \forall l \in \llbracket1,n\rrbracket
%	\end{equation}
%\end{assumption}
%Later (lemma \ref{"train-test-cond"}),\,we will show that,\,when using the standard cross %validation procedures,\,the training and validation masks verifies this condition.\\
%First,\,let's use proposition \ref{"Bernstein-extension"} to prove the following lemma:
%
%\begin{lemma}
%	\label{"RCV-supp"}
%	Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables, and $V_1,V_2,\dots V_K$ a sequence of masks that verifies assumption \ref{assum:mask-property} with size $n_V$.\,Moreover,\,suppose that assumption \ref{assum:hypo-class} and \ref{assum:cost-func} regarding the class $\mathcal{G}$ and $c$ hold.\,Define 
%	\begin{equation}\label{def:Z-CV}
%		Z=\ffrac{1}{K}\sum_{j=1}^{K}\sup_{g \in \mathcal{G}}\lvert \Tilde{\mathcal{R}}_{\alpha}(g,V_{j})-\mathcal{R}(g) \rvert,
%	\end{equation}
%	
% where $\Tilde{\mathcal{R}}_{\alpha}$ is defined by equation \ref{def:tilde-rcv}.\,Then the random variable $Z$  satisfies the Bernstein inequality	
%	
%	\[P\left(Z - E(Z) \geq t  \right)\leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).\]
%	
%\end{lemma}
%
%
%\begin{myproof}
% the reader is referred to appendix \ref{"lemma-RCV-supp-proof"}.
%	
%	
%\end{myproof}
%
%To obtain a probability bound of the estimate $Z$ via this lemma,\,one needs to control the term $E(Z)$.\,To do so, we will show a  result similar to lemma 14 in \cite{goix15}.
%\begin{lemma}
%	\label{"RCV-expectation"}
%        For any subsample $S\subset \{1,\ldots, n\}$ if size $n_S$ %mask $V$, and define
%	\[
%	Z'=\sup_{g \in \mathcal{G}} \bigg|\Tilde{\mathcal{R}}_{\alpha}(g,S)-\mathcal{R}(g)\bigg|.
%	\]
%	Then we have
%	\[
%	\EE(Z') \leq B(n_S,\alpha),
%	\]
%	with 
%\begin{equation}\label{"V-n-def"}
%  B(n_S,\alpha)= \ffrac{M\sqrt{\vapnikG}}{\sqrt{\alpha n_S}}
%%  {\color{red} + \frac{M_1  \vapnikG}{\alpha n_S}}
%\end{equation}  
%for some constant $M>0$.
%\end{lemma}
%
%\begin{myproof}
%	
%	See appendix \ref{"proof-RCv-expectation"}
%\end{myproof}
%
%
%Combining lemma \ref{"RCV-supp"} and lemma \ref{"RCV-expectation"} allows to deduce the following corollary. 
%
%\begin{corollary}
%	\label{"RCV-sup-control"}
%	Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables, and $V_1,V_2,\dots V_K$ a sequence of masks satisfying assumption \ref{assum:mask-property} .\, In addition suppose that assumption \ref{assum:hypo-class} and \ref{assum:cost-func} hold.\,then we have
%	\[P\left(Z - B(n_V,\alpha) \geq t \right)\leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right),\]
%	where $Z$ and $B$ are defined by equations \ref{def:Z-CV} and \ref{"V-n-def"} respectively.
%	
%\end{corollary}

%\begin{myproof} The idea is to show that $E(Z) \leq B(n_S,\alpha)$ and to conclude by using Lemma \eqref{"RCV-supp"}.\,To do so,\,notice that for 2 different masks  $V_{j}$ and $V_{j'}$ we have $\mathbb{E}\left[\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_j)- \mathcal{R}_{\alpha}(g)\bigg|\right]= \mathbb{E}\left[\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_{j'})- \mathcal{R}_{\alpha}(g)\bigg|\right]$ since all observations are i.i.d and the  vectors $V_j$'s have all the same length. Thus it follows that
%	\[\mathbb{E}\left[\ffrac{1}{K}\sum_{j=1}^K\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_j)- \mathcal{R}_{\alpha}(g)\bigg|\right]=
%	\mathbb{E}\left[\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_1)- \mathcal{R}_{\alpha}(g)\bigg|\right].\]
%	
%	
%	Now using Lemma  \ref{"RCV-expectation"} one obtains 
%	\[\underbrace{\mathbb{E}\left[\sup_{g \in \mathcal{G}}\bigg|\Tilde{\mathcal{R}}_{\alpha}(g,V_1)- \mathcal{R}_{\alpha}(g)\bigg|\right]}_{\mathbb{E}(Z) } \leq \underbrace{\ffrac{M\sqrt{\mathcal{V}_{\mathcal{G}}}}{\sqrt{n_{S}\alpha}}}_{B(n_{S},\alpha)}.\]
%	
%	Combining this with lemma \ref{"RCV-supp"} yields the desired result.  
%%	\[\PP(Z-B(n_{S},\alpha)\geq t) \leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right)\]
%\end{myproof}


%In order to use corollary \ref{"RCV-sup-control"} for a sequence  $V_{1:K}=(V_1,V_2,\dots,V_K)$, condition \eqref{"key-condition"}  must be checked.\,In the following lemma, we show that the classical cross validation procedures verifies assumption 4.
%
%\begin{lemma}
%	\label{"train-test-cond"}
%	For leave-one-out,\,leave-$p$-out,\,and $K$-fold procedures,\,the training samples 
%	$T_{1:K}$ and the validation samples $V_{1:K}$ satisfies assumption 4 i.e 
%	\begin{equation*}
%	\frac{1}{K}\sum_{j=1}^{K}\ffrac{\indic{l \in T_j} }{n_{T}}= \frac{1}{K}\sum_{j=1}^{K}\ffrac{\indic{l \in V_j} }{n_{V}}=\frac{1}{n} \quad \forall l \in \llbracket1,n\rrbracket.
%	\end{equation*}
%	
%\end{lemma}
%
%\begin{myproof}
%%	
%	Since the leave-one-out can be seen as a special case of $K$-fold, with $K=n$ it suffices to treat only the case of leave-$p$-out and $K$-fold .
%	
%	\paragraph{$K$-Fold.} For this procedure,\,the validation "masks" verifies the following property
%	\begin{equation}\label{"loo-k-fold-prop"}
%	\bigcup\limits_{j=1}^K V_j=\llbracket1,n\rrbracket \: and \: V_j\bigcap V_k=\varnothing\:, \:\forall j\neq k \in \llbracket1,K\rrbracket.
%	\end{equation}
%	
%	Under the hypothesis that $card(V_j)=n_{V}$  for all the validation sets, \eqref{"loo-k-fold-prop"} implies\,that
%	\begin{equation}
%	\label{"K-fold-equation"}
%	n=\sum_{j=1}^{K}card(V_j)=Kn_{V}. 
%	\end{equation}
%	
%	
%	Furthermore,\,under \eqref{"loo-k-fold-prop"},\,an index $l\in \llbracket 1,n \rrbracket$ belongs to a unique validation test $V_j'$ and to all the train sets $T_j=V_j^c$ with $j\neq j'$.\,Hence,\,we have
%	
%	\begin{equation*}
%	\begin{cases}
%	\sum_{j=1}^{K}\indic{l \in T_j} = K-1, \\
%	\sum_{j=1}^{K}\indic{l \in V_j} = 1.
%	\end{cases}  
%	\end{equation*}
%	Using \eqref{"K-fold-equation"} and the fact that $n_{T}=n-n_{V}=(K-1)n_{V}$ yields the desired result.
%%	
%%	\begin{equation*}
%%	\begin{cases}
%%	\ffrac{1}{Kn_{T}}\sum_{j=1}^{K}\indic{l \in T_j} = 1/n \\[10pt]
%%	\ffrac{1}{Kn_{V}}\sum_{j=1}^{K}\indic{l \in V_j} = 1/n,
%%	\end{cases}  
%%	\end{equation*}
%%	
%%	which is the desired result.
%	
%	\paragraph{Leave-$p$-out.}
%	In the leave-$p$-out procedure,\,the validation sets are all the subsamples of $\DD_n$ with $card(V_j)=p$,\,thus we have\,$K=\binom{n}{p}$. On the other hand,\,an index $l\in \llbracket 1,n \rrbracket$ belongs to $\binom{n-1}{p-1}$ validation sets.\,In fact, creating a $V_j$ such as $l \in V_j$ is equivalent to first picking $l$  and then choosing $m-1$  element from $\llbracket1,n\rrbracket \setminus \{l\}$.
%	Hence we have
%	
%	\begin{equation*}
%	\sum_{j=1}^{K}\indic{l \in V_j} = \binom{n-1}{p-1} \: \, , \: \forall l \in \llbracket1,n\rrbracket.
%	\end{equation*}
%	Recall that $n\binom{n-1}{p-1}=p\binom{n}{p}$ which yields 
%	\[\ffrac{1}{Kn_{V}}\sum_{j=1}^{K}\indic{l \in V_j}= \ffrac{1}{p\binom{n}{p}}\sum_{j=1}^{K}\indic{l \in V_j}= 1/n. \]
%	
%	Similar arguments can be used for the sequence $T_{1:K}$,\,and the proof is complete.
%	
%	\begin{remark*}
%		For the $K$-fold  cross validation,\,the hypothesis $card(V_j)=n_{V}$ where $n_{V}$ is independent of $j$   only holds when $n$ is divisible by $K$. But even when $K$  does not divide $n$,\, one can obtain still similar results to those presented in this paper  by straightforward modifications of the proofs.
%	\end{remark*}
%\end{myproof}

%Combining corollary \ref{"RCV-sup-control"} and lemma \ref{"train-test-cond"} gives the following proposition.
%
%
%\begin{prop}\label{"key-proposition-CV"} 
%	Let $\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ be a sequence of random variables.\,For leave-one-out,\,leave-$p$-out,\,and $K$-fold procedures we have  
%	\[\PP(Z-B(n_{V},\alpha)\geq t) \leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right). \] 
%	%
%%\quad \text{for } S_{1:K} \in \{T_{1:K},V_{1:K}\} \]
%	
%	where we recall that  $Z=\ffrac{1}{K}\sum_{j=1}^{K}\sup_{g \in \mathcal{G}}\lvert \Tilde{\mathcal{R}}_{\alpha}(g,S_{j})-\mathcal{R}(g) \rvert$.
%	% and $n_S=card(S_1)$.	
%\end{prop}

\subsection{Technical results}\label{sec:technicalResults}

\begin{lemma}\label{"RCV-ge-RN"}
Let $\Psi_{\alpha}$ be the ERM rule on the tail region of level $1-\alpha$ defined in (\ref{"g_alpha_j_def"}). Given a dataset	$\DD_n=(O_1,O_2,\dots,O_n)\in \mathcal{X}^n$ and a sequence of mask $V_{1:K}$ it holds that
\[   
\widehat{ \mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),S_n) \leq  \widehat{\mathcal{R}}_{CV,\alpha}(\Psi_{\alpha},V_{1:K}).
\]
In other words the \CV risk estimate of the ERM rule cannot be less than the empirical risk evaluated on the full dataset. 
\end{lemma}


\begin{proof}
The argument for $\alpha\neq 1$ is the same as the one for
 $\alpha=1$ (standard ERM) which may be found in \cite{kearns1999algorithmic}. We reproduce
  it for the sake of completeness. By definition of
  $\Psi_{\alpha}(S_n)$,\,one has

\begin{equation*}
  \forall j \in \llbracket 1,n \rrbracket \:,\: \widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(T_j),S_n) \geq \widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),S_n).
\end{equation*}

Since $\widehat{\mathcal{R}}_{\alpha}(g,S_n)= \ffrac{1}{n}\left( n_{V}\widehat{\mathcal{R}}_{\alpha}(g,V_j)+n_{T}\widehat{\mathcal{R}}_{\alpha}(g,T_j) \right)$, for $g\in \mathcal{G}$.\,It follows that
\begin{align*}
	\ffrac{1}{n}\left( n_{V}\underbrace{\widehat{\mathcal{R}}_{\alpha}(\Psi_\alpha(T_j),V_j)}_{\text{validation error}}+n_{T}\underbrace{\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(T_j),T_j)}_{\text{training error}}  \right) \geq \ffrac{1}{n}\big( n_{V}\widehat{\mathcal{R}}_{\alpha}(&\Psi_{\alpha}(S_n),V_j)\\& +  n_{T}\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),T_j) \big).
\end{align*}


Since $\Psi_{\alpha}(T_j)$ minimizes the training error on the $j$'th train set $T_j$, in particular we have $$\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),T_j) \geq  \widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(T_j),T_j),$$ hence %it follows that
\begin{equation}\label{ineq:cv-er-base}
	\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),V_j) \leq  \widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(T_j),V_j)\:,\:\forall j \in \llbracket 1 , K \rrbracket.
\end{equation}

In addition the average empirical risk of $\Psi_\alpha(S_n)$ is equal to its empirical risk on the full dataset, indeed
\begin{align*}
	\ffrac{1}{K}\bigg(\sum_{j=1}^{K}\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),V_j)\bigg)&=\ffrac{1}{Kn_{V}}\bigg(\sum_{j=1}^{K}\sum_{i\in V_j} c\big(\Psi_{\alpha}(S_n),O_i)\un{\lVert X_{i}\rVert>\lVert X_{(\lfloor \alpha n \rfloor\big)}\rVert }\bigg)\\
	&=\ffrac{1}{Kn_{V}}\bigg(\sum_{j=1}^{K}\sum_{i=1}^{n}c\big(\Psi_{\alpha}(S_n),O_i\big)\un{i \in V_j}\un{\lVert X_{i}\rVert>\lVert X_{(\lfloor \alpha n \rfloor)}\rVert }\bigg)\\
	&=\ffrac{1}{Kn_{V}}\bigg(\sum_{i=1}^{n}c\big(\Psi_{\alpha}(S_n),O_i\big)\un{\lVert X_{i}\rVert>\lVert X_{(\lfloor \alpha n \rfloor)}\rVert }\bigg)\sum_{j=1}^{K}\un{i \in V_j}\\
	(\text{By lemma }\ref{"train-test-cond"})&=\widehat{\mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n)).
\end{align*}

Thus \,by averaging inequality \ref{ineq:cv-er-base}, we get
\[   
\widehat{ \mathcal{R}}_{\alpha}(\Psi_{\alpha}(S_n),S_n) \leq  \widehat{\mathcal{R}}_{CV,\alpha}(\Psi_{\alpha},V_{1 : K}).
\]
\end{proof}
The following lemma is used in the proof of our second main result concerning \lpo risk estimation, see inequality~(\ref{eq:keyTheorem2fromLemma}). It is a generalization of  Markov inequality that is particularly useful for  cross-validation estimates. Our proof shares similarities with the proof of Theorem 4.1 in~\cite{kearns1999algorithmic} formulated under general algorithmic stability assumptions. 
\begin{lemma}\label{"RCV-markov"}
In the setting of Theorem \ref{theo:main-sanity-rare}, we have 
\begin{align*}
	\PP(\rcvEx(\Psi_{\alpha},V_{1 : K}) - \mathcal{R}_{CV,\alpha}(\Psi_{\alpha},V_{1 : K})  \geq &t ) \leq \\
	&\ffrac{\EE(\DevExt+\BiasCV+\abs{ \hat\risk_\alpha(\Psi_{\alpha}(S_n),S_n) - \risk_\alpha(\Psi_{\alpha}(S_n)) })}{t},
\end{align*}

where  $\BiasCV$ (resp $\DevExt$) is defined by equation \ref{"bias_CV"} (resp \ref{"dev_ext"}).
\end{lemma}

\begin{proof}
Set 
$\rcvEx=\rcvEx(\Psi_{\alpha},V_{1 : K})$, $\mathcal{R}_{CV,\alpha}=\mathcal{R}_{CV,\alpha}(\Psi_{\alpha},V_{1 : K})$ , $  \hat\risk_\alpha=\hat\risk_\alpha(\Psi_{\alpha}(S_n),S_n)$, $ \risk_\alpha=\risk_\alpha(\Psi_{\alpha}(S_n))$.\\
 For any integrable real valued random variable $W$, and any $t>0$ write  
  $$\EE[W]= \PP[W\ge t]\EE[W \,|\, W\ge t] + \EE[W \un{W<t}].$$ Reorganising, we obtain the following generalized Markov inequality, 
  \[
    \PP[W>t] = \frac{\EE[W] - \EE[W \un{W<t}]}{\EE[W \,|\, W\ge t]}
    \le \frac{\EE(W) - \EE(W \un{W<t})}{t}. 
  \]
  Letting $W = \rcvEx-\mathcal{R}_{CV,\alpha}$ we obtain
%     \begin{equation*}
%      \begin{split}
% \EE(\rcvEx-\mathcal{R}_{CV,\alpha})=\PP(\rcvEx&-\mathcal{R}_{CV,\alpha}\geq t)\EE(\rcvEx-\mathcal{R}_{CV,\alpha} \mid \rcvEx-\mathcal{R}_{CV,\alpha} \geq t)\\&+\EE\left[(\rcvEx-\mathcal{R}_{CV,\alpha}) \indic{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right].
% \end{split}
% \end{equation*} 
% Thus one obtains 
\begin{equation}
\label{"exp-CV-one"}
\PP(\rcvEx-\mathcal{R}_{CV,\alpha}\geq t)= \frac{\EE(\rcvEx-\mathcal{R}_{CV,\alpha})-\EE\left[(\rcvEx-\mathcal{R}_{CV,\alpha}) \un{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right]}{t}.
\end{equation} 


Using the fact that $\EE(\tilde{\mathcal{R}}_{CV,\alpha}-\risk_{CV,\alpha})=0$ and that $\DevExt=\abs{\rcvEx-\tilde{\mathcal{R}}_{CV,\alpha}}$, one gets
\begin{align}
\EE(\rcvEx-\mathcal{R}_{CV,\alpha})&=\EE(\rcvEx-\tilde{\mathcal{R}}_{CV,\alpha}) \nonumber \\ &\leq \EE(\DevExt).
\label{"exp-CV-two"}
\end{align} 
Now using lemma  \ref{"RCV-ge-RN"} write

\begin{align}
\EE\left[(\mathcal{R}_{CV,\alpha}-\rcvEx) \ind_{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right] &\leq \EE\left[(\mathcal{R}_{CV,\alpha}-\widehat\risk_\alpha) \ind_{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right] \nonumber \\ & \leq \EE\left[\abs{\mathcal{R}_{CV,\alpha}-\widehat\risk_\alpha} \ind_{\rcvEx-\mathcal{R}_{CV,\alpha} \leq t} \right]  \nonumber \\ & 
\leq  \EE\left[\abs{\mathcal{R}_{CV,\alpha}-\widehat\risk_\alpha} \right] \nonumber \\ &
\leq \EE\left[\abs{\mathcal{R}_{CV,\alpha}-\risk_\alpha} \right]+ \EE\left[\abs{\risk_\alpha-\widehat\risk_\alpha} \right] \nonumber \\
&=\EE\left[\BiasCV \right]+ \EE\left[\abs{\risk_\alpha-\widehat\risk_\alpha} \right].
\label{"exp-CV-three"}
\end{align}

The last line follows from the definition of $\BiasCV$ in (\ref{"bias_CV"}). Combining inequality \eqref{"exp-CV-one"} with equations \eqref{"exp-CV-two"} and \eqref{"exp-CV-three"} yields
	\[\PP(\rcvEx-\mathcal{R}_{CV,\alpha} \geq t ) \leq \ffrac{\EE(\DevExt+\BiasCV+\abs{\hat\risk_\alpha- \risk_{\alpha}})}{t}, \]
which concludes the proof.
\end{proof}

To conclude this section, we extend Theorem~10 in~\cite{goix15} bounding the supremum deviations of the empirical measure on low probability regions, to handle the case of any cost function $c$ absolutely bounded by one.
\begin{lemma}\label{lemma:inv-goix}
Recall the definitions of the risk $\risk_\alpha$ and its empirical version $\ER_\alpha$ given in Section~\ref{sec:framework} and introduce the (random) supremum deviations 
		\[Z'=\sup_{g \in \mathcal{G}}\lvert \widehat{\mathcal{R}}_{\alpha}(g,S_n)-\mathcal{R}_\alpha(g) \rvert.\]
If $\mathcal{G}$ is a family of classifiers with finite VC-dimension and $c$ a bounded cost function with $\sup_{g,o}|c(g,o)|\le 1$, then,  the following Bernstein-type  inequality holds, 
	\[ \PP(Z'-Q(n,\alpha) \geq t)\leq 3\exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right), \]
	where $Q(n,\alpha)=B(n,\alpha)+\ffrac{1}{n\alpha}$ and $B$ is defined by
        %
        % equation \ref{"V-n-def"}.
\begin{equation}\label{"V-n-def"}
  B(n,\alpha) = \ffrac{M\sqrt{\vapnikG}}{\sqrt{\alpha n}} %  {\color{red} + \frac{M_1  \vapnikG}{\alpha n_S}},
\end{equation}  
and $M$ is a universal constant. 
        
\end{lemma}

\begin{proof}
	Write $Z' \leq Z_1 +Z_2$ with :
	\[Z_1=\sup_{g \in \mathcal{G}}\lvert \widehat{\mathcal{R}}_{\alpha}(g,S_n)-\Tilde{\mathcal{R}}_{\alpha}(g,S_n) \rvert,\]
	\[ Z_2=\sup_{g \in \mathcal{G}}\lvert\Tilde{\mathcal{R}}_{\alpha}(g,S_n)-\mathcal{R}_{\alpha}(g)\rvert.\]
Concerning $Z_2$, applying Corollary \ref{"RCV-sup-control"} with $K=1$ , $V_1=S_n$, $\mathcal{A}=(\lVert X \rVert \geq t_\alpha)$, yields
		\begin{equation}\label{ineq:Z-1-UB}
	\PP(Z_2 - B(n,\alpha) \geq t) \leq \exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).
	\end{equation}
We now focus on $Z_1$. Define 
$$u_{i}=\left|\un{\lVert X_{i}\rVert>\lVert X_{(\lfloor \alpha n \rfloor)}\rVert}
-\un{\lVert X_{i} \rVert \geq t_\alpha}\right|$$ 
and notice that $ Z_1\leq \ffrac{1}{n\alpha}\sum_{i=1}^{n}u_{i}$. It is known (see for instance the bound for the term $A$ in \cite{jalalzai2018binary}, page 12) that 
\begin{equation*}
\ffrac{1}{n\alpha}\sum_{i=1}^{n}u_{i}\leq  \frac{1}{\alpha}\left|\frac{1}{n}\sum_{i= 1}^n \un{\lVert X\rVert \geq t_\alpha}-\alpha\right| + \frac{1}{n\alpha}. 
\end{equation*}
Now,  by noticing that $\Var(\indic{\lVert X\rVert \geq t_\alpha}) \le \alpha$ and using Bernstein's inequality, we get
\begin{align*}
\PP\left(\bigg|\frac{1}{n}\sum_{i= 1}^n \indic{\lVert X\rVert \geq t_\alpha}-\alpha \bigg|\geq t\right)&\leq 2\exp\left(\ffrac{-n t^2}{2(\alpha+t/3)}\right)\\&\leq 2\exp\left(\ffrac{-n t^2}{2(4\alpha+t/3)}\right).
\end{align*}
Finally,\,dividing by $\alpha$, we get 
% and noticing that  $P(\abs{X}\geq t) \leq P(X\geq t)+ P(-X\geq t) $ leads to 
\begin{align*}
\PP(\frac{1}{\alpha}&\bigg|\sum_{i= 1}^n \frac{1}{n}\indic{\lVert X\rVert \geq t_\alpha}-\alpha\bigg| \geq t)\leq 2\exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).
\end{align*}
Therefore we finally obtain
\begin{equation}\label{bound:z1}
\PP\left(  \ffrac{1}{n\alpha}\sum_{i=1}^{n}u_{i} - 1/n\alpha  \geq t \right) \leq  2\exp\left(\ffrac{-n\alpha t^2}{2(4+t/3)}\right).
\end{equation}
The result follows using $Z' \leq Z_1 + Z_2$ and $ Z_1\leq \ffrac{1}{n\alpha}\sum_{i=1}^{n}u_{i}$.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_crossval.tex"
%%% End:

